Observation of the Crab Nebula with the HAWC Gamma-Ray Observatory

The Crab Nebula is the brightest TeV gamma-ray source in the sky and has been used for the past 25 years as a reference source in TeV astronomy, for calibration and verification of new TeV instruments. The High Altitude Water Cherenkov Observatory (HAWC), completed in early 2015, has been used to observe the Crab Nebula at high significance across nearly the full spectrum of energies to which HAWC is sensitive. HAWC is unique for its wide field-of-view, nearly 2 sr at any instant, and its high-energy reach, up to 100 TeV. HAWC's sensitivity improves with the gamma-ray energy. Above $\sim$1 TeV the sensitivity is driven by the best background rejection and angular resolution ever achieved for a wide-field ground array. We present a time-integrated analysis of the Crab using 507 live days of HAWC data from 2014 November to 2016 June. The spectrum of the Crab is fit to a function of the form $\phi(E) = \phi_0 (E/E_{0})^{-\alpha -\beta\cdot{\rm{ln}}(E/E_{0})}$. The data is well-fit with values of $\alpha=2.63\pm0.03$, $\beta=0.15\pm0.03$, and log$_{10}(\phi_0~{\rm{cm}^2}~{\rm{s}}~{\rm{TeV}})=-12.60\pm0.02$ when $E_{0}$ is fixed at 7 TeV and the fit applies between 1 and 37 TeV. Study of the systematic errors in this HAWC measurement is discussed and estimated to be $\pm$50\% in the photon flux between 1 and 37 TeV. Confirmation of the Crab flux serves to establish the HAWC instrument's sensitivity for surveys of the sky. The HAWC survey will exceed sensitivity of current-generation observatories and open a new view of 2/3 of the sky above 10 TeV.

==> authors.tex <==
\author{
A.U.~Abeysekara\altaffilmark{1},
A.~Albert\altaffilmark{2},
R.~Alfaro\altaffilmark{3},
C.~Alvarez\altaffilmark{4},
J.D.~\'{A}lvarez\altaffilmark{5},
R.~Arceo\altaffilmark{4},
J.C.~Arteaga-Vel\'{a}zquez\altaffilmark{5},
H.A.~Ayala Solares\altaffilmark{6},
A.S.~Barber\altaffilmark{1},
N.~Bautista-Elivar\altaffilmark{7},
A.~Becerril\altaffilmark{3},
E.~Belmont-Moreno\altaffilmark{3},
S.Y.~BenZvi\altaffilmark{8},
D.~Berley\altaffilmark{9},
J.~Braun\altaffilmark{10},
C.~Brisbois\altaffilmark{6},
K.S.~Caballero-Mora\altaffilmark{4},
T.~Capistr\'{a}n\altaffilmark{11},
A.~Carrami\~{n}ana\altaffilmark{11},
S.~Casanova\altaffilmark{12},
M.~Castillo\altaffilmark{5},
U.~Cotti\altaffilmark{5},
J.~Cotzomi\altaffilmark{13},
S.~Couti\~{n}o de Le\'{o}n\altaffilmark{11},
E.~de la Fuente\altaffilmark{14},
C.~De Le\'{o}n\altaffilmark{13},
T.~DeYoung\altaffilmark{15},
B.L.~Dingus\altaffilmark{2},
M.A.~DuVernois\altaffilmark{10},
J.C.~D\'{i}az-V\'{e}lez\altaffilmark{14},
R.W.~Ellsworth\altaffilmark{16},
D.W.~Fiorino\altaffilmark{9},
N.~Fraija\altaffilmark{17},
J.A.~Garc\'{i}a-Gonz\'{a}lez\altaffilmark{3},
M.~Gerhardt\altaffilmark{6},
A.~Gonz\'{a}lez Mu\"{n}oz\altaffilmark{3},
M.M.~Gonz\'{a}lez\altaffilmark{17},
J.A.~Goodman\altaffilmark{9},
Z.~Hampel-Arias\altaffilmark{10},
J.P.~Harding\altaffilmark{2},
S.~Hernandez\altaffilmark{3},
A.~Hernandez-Almada\altaffilmark{3},
J.~Hinton\altaffilmark{18},
C.M.~Hui\altaffilmark{19},
P.~H\"{u}ntemeyer\altaffilmark{6},
A.~Iriarte\altaffilmark{17},
A.~Jardin-Blicq\altaffilmark{18},
V.~Joshi\altaffilmark{18},
S.~Kaufmann\altaffilmark{4},
D.~Kieda\altaffilmark{1},
A.~Lara\altaffilmark{20},
R.J.~Lauer\altaffilmark{21},
W.H.~Lee\altaffilmark{17},
D.~Lennarz\altaffilmark{22},
H.~Le\'{o}n Vargas\altaffilmark{3},
J.T.~Linnemann\altaffilmark{15},
A.L.~Longinotti\altaffilmark{11},
G.~Luis Raya\altaffilmark{7},
R.~Luna-Garc\'{i}a\altaffilmark{23},
R.~L\'{o}pez-Coto\altaffilmark{18},
K.~Malone\altaffilmark{24},
S.S.~Marinelli\altaffilmark{15},
O.~Martinez\altaffilmark{13},
I.~Martinez-Castellanos\altaffilmark{9},
J.~Mart\'{i}nez-Castro\altaffilmark{23},
H.~Mart\'{i}nez-Huerta\altaffilmark{25},
J.A.~Matthews\altaffilmark{21},
P.~Miranda-Romagnoli\altaffilmark{26},
E.~Moreno\altaffilmark{13},
M.~Mostaf\'{a}\altaffilmark{24},
L.~Nellen\altaffilmark{27},
M.~Newbold\altaffilmark{1},
M.U.~Nisa\altaffilmark{8},
R.~Noriega-Papaqui\altaffilmark{26},
R.~Pelayo\altaffilmark{23},
J.~Pretz\altaffilmark{24},
E.G.~P\'{e}rez-P\'{e}rez\altaffilmark{7},
Z.~Ren\altaffilmark{21},
C.D.~Rho\altaffilmark{8},
C.~Rivi\`{e}re\altaffilmark{9},
D.~Rosa-Gonz\'{a}lez\altaffilmark{11},
M.~Rosenberg\altaffilmark{24},
E.~Ruiz-Velasco\altaffilmark{3},
H.~Salazar\altaffilmark{13},
F.~Salesa Greus\altaffilmark{12},
A.~Sandoval\altaffilmark{3},
M.~Schneider\altaffilmark{28},
H.~Schoorlemmer\altaffilmark{18},
G.~Sinnis\altaffilmark{2},
A.J.~Smith\altaffilmark{9},
R.W.~Springer\altaffilmark{1},
P.~Surajbali\altaffilmark{18},
I.~Taboada\altaffilmark{22},
O.~Tibolla\altaffilmark{4},
K.~Tollefson\altaffilmark{15},
I.~Torres\altaffilmark{11},
T.N.~Ukwatta\altaffilmark{2},
L.~Villase\~{n}or\altaffilmark{5},
T.~Weisgarber\altaffilmark{10},
S.~Westerhoff\altaffilmark{10},
I.G.~Wisher\altaffilmark{10},
J.~Wood\altaffilmark{10},
T.~Yapici\altaffilmark{15},
G.B.~Yodh\altaffilmark{29},
P.W.~Younk\altaffilmark{2},
A.~Zepeda\altaffilmark{25},
H.~Zhou\altaffilmark{2}
}
\affil{$^{1}$ Department of Physics and Astronomy, University of Utah, Salt Lake City, UT, USA }
\affil{$^{2}$ Physics Division, Los Alamos National Laboratory, Los Alamos, NM, USA }
\affil{$^{3}$ Instituto de F\'{i}sica, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Ciudad de M\'{e}xico, M\'{e}xico }
\affil{$^{4}$ Universidad Aut\'{o}noma de Chiapas, Tuxtla Guti\'{e}rrez, Chiapas, M\'{e}xico}
\affil{$^{5}$ Universidad Michoacana de San Nicol\'{a}s de Hidalgo, Morelia, M\'{e}xico }
\affil{$^{6}$ Department of Physics, Michigan Technological University, Houghton, MI, USA }
\affil{$^{7}$ Universidad Politecnica de Pachuca, Pachuca, Hgo, M\'{e}xico }
\affil{$^{8}$ Department of Physics \& Astronomy, University of Rochester, Rochester, NY , USA }
\affil{$^{9}$ Department of Physics, University of Maryland, College Park, MD, USA }
\affil{$^{10}$ Department of Physics, University of Wisconsin-Madison, Madison, WI, USA }
\affil{$^{11}$ Instituto Nacional de Astrof\'{i}sica, \'{O}ptica y Electr\'{o}nica, Puebla, M\'{e}xico }
\affil{$^{12}$ Instytut Fizyki Jadrowej im Henryka Niewodniczanskiego Polskiej Akademii Nauk, IFJ-PAN, Krakow, Poland }
\affil{$^{13}$ Facultad de Ciencias F\'{i}sico Matem\'{a}ticas, Benemérita Universidad Aut\'{o}noma de Puebla, Puebla, M\'{e}xico }
\affil{$^{14}$ Departamento de F\'{i}sica, Centro Universitario de Ciencias Exactas e Ingenierias, Universidad de Guadalajara, Guadalajara, M\'{e}xico }
\affil{$^{15}$ Department of Physics and Astronomy, Michigan State University, East Lansing, MI, USA }
\affil{$^{16}$ School of Physics, Astronomy, and Computational Sciences, George Mason University, Fairfax, VA, USA }
\affil{$^{17}$ Instituto de Astronom\'{i}a, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Ciudad de M\'{e}xico, M\'{e}xico }
\affil{$^{18}$ Max-Planck Institute for Nuclear Physics, 69117 Heidelberg, Germany}
\affil{$^{19}$ NASA Marshall Space Flight Center, Astrophysics Office, Huntsville, AL 35812, USA}
\affil{$^{20}$ Instituto de Geof\'{i}sica, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Ciudad de M\'{e}xico, M\'{e}xico }
\affil{$^{21}$ Dept of Physics and Astronomy, University of New Mexico, Albuquerque, NM, USA }
\affil{$^{22}$ School of Physics and Center for Relativistic Astrophysics - Georgia Institute of Technology, Atlanta, GA, USA 30332 }
\affil{$^{23}$ Centro de Investigaci\'{o}n en Computaci\'{o}n, Instituto Polit\'{e}cnico Nacional, Ciudad de M\'{e}xico, M\'{e}xico}
\affil{$^{24}$ Department of Physics, Pennsylvania State University, University Park, PA, USA }
\affil{$^{25}$ Physics Department, Centro de Investigaci\'{o}n y de Estudios Avanzados del IPN, Ciudad de M\'{e}xico, DF, M\'{e}xico }
\affil{$^{26}$ Universidad Aut\'{o}noma del Estado de Hidalgo, Pachuca, M\'{e}xico }
\affil{$^{27}$ Instituto de Ciencias Nucleares, Universidad Nacional Aut\'{o}noma de M\'{e}xico, Ciudad de M\'{e}xico, M\'{e}xico }
\affil{$^{28}$ Santa Cruz Institute for Particle Physics, University of California, Santa Cruz, Santa Cruz, CA, USA }
\affil{$^{29}$ Department of Physics and Astronomy, University of California, Irvine, Irvine, CA, USA }

